CoNewsReader: Supporting Comprehensive Understanding and Raising Critical Thoughts on Social Media News Through Comments

Critical news reading (CNR), which requires grasping the holistic ideas of and raising critical thoughts on the news, is beneficial yet challenging for general people who usually get information on daily social media. Comments under the news can aid CNR by providing complementary information and other readers' diverse and critical thoughts. However, it is under-investigated how to leverage these comments to support users in CNR. In this paper, we first derive user requirements for a comment-based CNR tool from literature and a formative study (N=12). Then, we develop CoNewsReader, a comment-based interactive CNR tool powered by a large language model. CoNewsReader supports users in grasping the news idea with complementary information from comments, filtering useful comments for CNR, and getting questions generated based on the comments to conduct critical thinking. Our within-subjects study with 24 university students indicates that compared to a baseline news reading interface in social media, participants with CoNewsReader have a more engaging CNR experience and perform better on comprehending the news and raising critical thoughts. We discuss design considerations for supporting reading tasks with user- and machine-generated content.

==> Tabel/Data_mann.tex <==
\begin{table*}
\centering
\begin{tabular}{ccccccc} 
\hline
\multirow{2}{*}{Category}   & \multirow{2}{*}{Factor} & \Toolname{} & Baseline  & \multicolumn{3}{c}{Statistics}  \\ 
\cline{5-7}
                            &                         & Mean/S.D.                    & Mean/S.D. & U    & p        & Sig.          \\ 
\hline
\multirow{7}{*}{Engagement} & Concentration           & 6.08/0.76                    & 5.25/1.16 & 42.5 & 0.081455 & ns            \\
                            & Sense of Ecstasy        & 6.00/1.22                    & 3.83/1.14 & 16   & 0.000884 & ***           \\
                            & Clarity                 & 5.75/0.92                    & 5.17/1.40 & 58   & 0.418635 &               \\
                            & Doability               & 4.75/1.88                    & 3.50/1.89 & 44.5 & 0.113636 &               \\
                            & Sense of Serenity       & 5.42/1.11                    & 4.33/1.25 & 39   & 0.05136  & ns            \\
                            & Timelessness Feeling    & 5.50/1.32                    & 4.92/1.44 & 52.5 & 0.252314 &               \\
                            & Intrinsic Motivation    & 6.00/0.91                    & 4.42/1.55 & 31   & 0.016194 & *             \\ 
\hline
\multirow{6}{*}{Workload}   & Mental Demand           & 4.17/1.46                    & 4.92/1.26 & 96   & 0.164495 &               \\
                            & Physical Demand         & 2.25/1.36                    & 2.50/1.44 & 78.5 & 0.718109 &               \\
                            & lemporal Demand         & 3.33/1.89                    & 4.25/1.92 & 91.5 & 0.259738 &               \\
                            & Performance             & 4.92/1.38                    & 4.17/1.21 & 47   & 0.147448 &               \\
                            & Effort                  & 4.17/1.86                    & 5.00/1.22 & 90   & 0.299142 &               \\
                            & Frustration             & 2.33/0.85                    & 3.33/1.37 & 104  & 0.062056 & ns            \\ 
\hline
\multirow{3}{*}{Acceptance} & Usefulness              & 5.83/1.11                    & 4.04/1.42 & 23.5 & 0.00546  & **            \\
                            & Easy to Use             & 5.48/1.16                    & 4.08/1.00 & 25   & 0.007084 & ***           \\
                            & Intention to use        & 5.33/1.52                    & 3.67/1.57 & 33.5 & 0.027218 & *             \\
\hline
\end{tabular}
\caption{}
\label{rq23table}
\end{table*}
